OPTWIN: Drift identification with optimal sub-windows

Online Learning (OL) is a field of research that is increasingly gaining attention both in academia and industry. One of the main challenges of OL is the inherent presence of concept drifts, which are commonly defined as unforeseeable changes in the statistical properties of an incoming data stream over time. The detection of concept drifts typically involves analyzing the error rates produced by an underlying OL algorithm in order to identify if a concept drift occurred or not, such that the OL algorithm can adapt accordingly. Current concept-drift detectors perform very well, i.e., with low false negative rates, but they still tend to exhibit high false positive rates in the concept-drift detection. This may impact the performance of the learner and result in an undue amount of computational resources spent on retraining a model that actually still performs within its expected range. In this paper, we propose OPTWIN, our "OPTimal WINdow" concept drift detector. OPTWIN uses a sliding window of events over an incoming data stream to track the errors of an OL algorithm. The novelty of OPTWIN is to consider both the means and the variances of the error rates produced by a learner in order to split the sliding window into two provably optimal sub-windows, such that the split occurs at the earliest event at which a statistically significant difference according to either the $t$- or the $f$-tests occurred. We assessed OPTWIN over the MOA framework, using ADWIN, DDM, EDDM, STEPD and ECDD as baselines over 7 synthetic and real-world datasets, and in the presence of both sudden and gradual concept drifts. In our experiments, we show that OPTWIN surpasses the F1-score of the baselines in a statistically significant manner while maintaining a lower detection delay and saving up to 21% of time spent on retraining the models.

==> Sections/2.Background_RelatedWorks.tex <==
\section{Background \& Related Works}

We next formally introduce the problem of concept drift and review its principal characteristics (cf. Section \ref{sec:background}). We also discuss the most important related approaches for concept-drift detection from the literature, which serve as inspiration and baselines of our work throughout this paper (cf. Section \ref{sec:related-works}).

\subsection{Background}
\label{sec:background}

%\textbf{Overview of concept drift research: source of drift, concept drift type, drift understanding, and drift adaptation strategy.} 
A concept drift may exhibit different characteristics whose understanding is essential for a fast and reliable detection. %Below, we present its formal definition. %Then, we explain the different concept drift sources. Next, we describe the concept drift types. Later, we present the strategies used to adapt and recover from a concept drift. Last, we show how to evaluate concept-drift detectors.  
%\textbf{Formal concept drift definition}
Consider an unbounded data stream that receives {\em features} $x_i \in X$ and {\em labels} $y_i \in Y$ in the form of pairs of instances $(x_i,y_i)$. At {\em time} $t$, these instances follow a certain distribution $P_t(X,Y)$. A concept drift is the change of this distribution over time. Formally, a concept drift occurs at time $t+1$ iff $P_t(X,Y) \neq P_{t+1}(X,Y)$ \cite{lu2016concept, lu2018learning, gama2014survey}. 
%\textbf{Explain the source of the drift.}
The underlying data distribution $P_t(X,Y)$ may also be decomposed and expressed as a product of probabilities $P_t(X,Y) = P_t(X) \times P_t(Y|X)$ via the well-known {\em chain rule of probability}. Thus, a concept drift may come from two {\em sources}: (1) $P_t(X) \neq P_{t+1}(X)$, which is known as a {\em virtual drift} because it does not impact the decision boundaries of the learner; and (2) $P_t(Y|X) \neq P_{t+1}(Y|X)$, which is known as an {\em actual drift} because it directly impacts the learner's accuracy \cite{lu2016concept, lu2018learning, gama2014survey}. It is also possible to have both drift sources simultaneously \cite{lu2018learning}.

%\textbf{Explain drift type.}
Another important characteristic of a concept drift is its {\em type}. Concept drifts can be (1) {\em sudden}; (2) {\em incremental}; (3) {\em gradual}; and (4) {\em reoccurring} (see Figure \ref{fig:drift-type}) \cite{lu2018learning,gama2014survey}. Sudden drifts occur when the probability distribution changes completely within a single step. Incremental drifts occur when the distribution $P_t(X,Y)$ changes incrementally until its convergence. Gradual drifts occur when the new distribution gradually replaces the old one. Reoccurring drifts occur when distributions can reoccur after some time. 
\begin{figure}[ht]
  \centering
  \vspace{-2mm}
  \includesvg[width=0.5\textwidth]{Figures/drift-type.svg}
  \vspace{-2mm}
  \caption{Concept drift types.}
  \label{fig:drift-type}
\end{figure}

%\textbf{Explain drift adaptation strategies.}
To recover from concept drifts, one may adapt the learner according to two main strategies: (1) {\em active drift adaptation}, which triggers drift adaptation only after a concept drift is flagged by the drift detector; and (2) {\em passive drift adaptation}, in which the learner is constantly adapting itself, independently of the detection of drifts \cite{heusinger2020passive}. The active drift-adaptation strategy depends on the correct identification of the drifts but avoids spending computational resources and time on (re-)training a learner that has already converged. Therefore, we further focus on the active drift-adaptation strategy in the following. 

 %\textbf{Explain drift adaptation strategies. - active drift adaptation}
 There are many sub-strategies for active drift adaptation. The selection of the appropriate one depends not only on the type and source of the drifts but also on the use-case and the adopted learner. A common strategy is to train a new model with the latest data points whenever a drift is identified. Another strategy is to adjust the current learner instead of training a new one from scratch. Moreover, it is also possible to have an ensemble of learners, which is primarily useful for adapting to reoccurring drifts \cite{lu2018learning}. 

%\textbf{Explain how to evaluate concept drifts.}
The most popular procedure to evaluate learning algorithms that handle concept drifts is the {\em prequential procedure}. Prequential is an evaluation scheme in which each data point is used for testing before training the learning algorithm. Therefore, it is not necessary to know when a drift occurred to perform the evaluation, which is useful when using real-world datasets that do not have labeled drifts \cite{lu2018learning}. Regarding the metrics used to evaluate the drift detector, one may refer to the following ones: TPs, FPs and FNs (and hence {\em precision}, {\em recall} and {\em F1-score}) in the detection rates, as well as the {\em delay} of the detection \cite{lu2018learning, dasu2006information}.

\subsection{Related Works}
\label{sec:related-works}

%\textbf{ADWIN}
%\smallskip
\noindent\textbf{ADWIN} \cite{bifet2007learning} (for ``ADaptive WINdowing'') is an algorithm with a sliding window $W$ that takes as input a confidence level $\delta \in (0,1)$ and an unbounded sequence of real values $X=\langle x_1, x_2, ..., x_i, ... \rangle$ from a data stream. Each input $x_i$ is expected to be in $[0,1]$ and is stored in a finite window $W\subset X$. The idea of the algorithm is that a concept drift occurs whenever there are two subsequent sub-windows of $W$ with an average difference in their mean above $\epsilon_{cut}$, which is guaranteed to yield a {\em confidence level} of $\delta$. %It is based on the common T-test \cite{t-test} for paired samples and is guaranteed to yield a {\em confidence level} of $\delta$ at which it makes the cut. 
If a drift is detected, a part of $W$ is dropped, and the algorithm is ready to resume the drift detection. ADWIN has guaranteed bounds on all error distributions. However, the observed errors usually tend to follow a normal distribution. Thus, they tightened their $\epsilon_{cut}$ accordingly and evaluated the algorithm taking those new bounds. Furthermore, as ADWIN checks multiple sub-windows of $W$, its complexity is $\mathcal{O}(\log{}|W|)$ per iteration (where an iteration is ideally triggered for each new element that arrives from the stream).

%\textbf{DDM}
%\smallskip
\noindent\textbf{DDM} \cite{gama2004learning} (for ``Drift Detection Method'') also receives as parameter a value $\delta$ related to the confidence level of the algorithm, and a sequence of data instances $X$ which are available one by one from a data stream. However, the data stream is expected to follow a binomial distribution, as its values represent the number of errors in a sample of $n$ instances. Therefore, it is primarily suited for classification problems rather than for regression. The main idea of DDM is that, as the number of samples increases, the number of errors from a learner will decrease. Therefore, if the error rate from the learner increases above a certain threshold, it means that a concept drift occurred. Thus, DDM tracks the minimal error rate $p_{min}$ from $X$ and its respective standard deviation $s_{min}$. Then, DDM flags a drift at step $i \geq 30$ iff $p_i + s_i \geq p_{min} + \delta s_{min}$. When a drift is detected, the algorithm is reset. One advantage of DDM is its lightweight nature due to storing only $p_{min}$ and $s_{min}$. However, DDM is known for its decreased performance when detecting slow gradual changes. 

%\textbf{EDDM}
%\smallskip
\noindent\textbf{EDDM} \cite{baena2006early} (for ``Early Drift Detection Method'') is similar to DDM but uses the distance between errors to identify concept drifts. Therefore, EDDM is suited only for binary input data, which does not allow it to be used for regression problems. They assume that, as the number of examples increases, the distance between errors will increase accordingly. Therefore, if this distance decreases more than a threshold, a concept drift is flagged. Thus, EDDM tracks the maximum distance between errors $p_{max}'$ and its respective standard deviation $s_{max}'$. Then, after analyzing at least 30 errors, EDDM flags a drift at step $t$ if $(p_{t}' + 2\,s_{t}') / (p_{max}' + 2\,s_{max}' < \delta)$, with $\delta$ again representing a simple form of confidence level for the detected concept drifts. According to the authors, EDDM improves DDM's performance when identifying gradual concept drifts while maintaining good performance on sudden drifts. 

%\textbf{STEPD}
%\smallskip
\noindent\textbf{STEPD} \cite{nishida2007detecting} (for using the ``Statistical Test of Equal Proportions'') is a lightweight drift detector that also considers a sequence of data instances $X$ as input. The idea of STEPD is that the recent accuracy of a learner shall be similar to its overall accuracy, otherwise a concept drift occurred. As the name suggests, STEPD checks the equality-of-proportions hypothesis test \cite{massey2006tests} by comparing the most recent values from $X$ (kept in a sliding window $W$) with the other values in $X$, thus comparing $X_{0:W}$ and $X_{W:|X|-1}$. It also considers that the data follows a normal distribution, and with a confidence level of $\delta$, it can determine if the null hypothesis is rejected and a concept drift is flagged. In this case, the algorithm is reset. The value of $W$ selected by the authors was 30. 

%\textbf{ECDD}
%\smallskip
\noindent\textbf{ECDD} \cite{ross2012exponentially} is the acronym for ``Exponentially Weighted Moving Average'' (EWMA) for concept-drift detection. It is a drift-detection method based on EWMA that checks the misclassification rate of its underlying learners. ECDD receives a sequence of data instances $X$ as input, which it assumes to follow a Bernoulli distribution. ECDD is suited only for classification problems, as it only accepts binary data from the data stream. Other than $X$, ECDD takes as inputs $ARL_0$, which is the time one expects between detecting false positives; and $\lambda$, which dictates how much weight new data has compared to the old one. Despite being computationally expensive to calculate, $ARL_0$ can be approximated before starting to process the data stream. ECDD then uses pre-calculated polynomials, $ARL_0$ and $\lambda$ to update its estimators. With its updated estimators, ECDD detects if a concept drift occurred or not. Finally, if a drift is detected, the algorithm is reset. 

%\smallskip
We note that all algorithms described above additionally have a form of warning detection which can be used to assist in the concept drift adaptation. The warning is usually a simple relaxation of the drift threshold which can be used to start training a new learner before the actual concept drift is flagged. %For example, one could have $\delta=0.99$ as the confidence level for the drift detection and $\delta'=0.95$ as the confidence level for the warning detection. In the case a concept drift is flagged after a warning was in place, instead of using a new learner after the concept drift is detected, it is possible to use one that has already been trained with the correct data distribution since the warning was flagged. This ``head start'' guarantees a better performance for the new learner. On the other hand, if the algorithm surpasses the warning threshold but does not reach the drift threshold (i.e., it then falls back below the warning threshold), the learner trained in the background is discarded (thus giving a false-positive warning). 


==> Sections/4.Experiments_Results.tex <==
\section{Experiments \& Results}
\label{sec:experiments}

%\textbf{Over view of the experiments.} 
In this section, we report our detailed experiments to asses OPTWIN. We compared OPTWIN to the most-commonly used baselines for concept-drift detection: ADWIN, DDM, EDDM, STEPD, and ECDD. We performed most of the experiments using the common MOA \cite{DBLP:moa} framework which is a Java-based data stream simulator. In addition, we performed experiments on Python to asses OPTWIN on a Neural Network (NN) use case, which would not be possible via MOA. 

\subsection{MOA Experiments}
%\textbf{Overview of setting used on MOA.} 
We compared 3 configurations of OPTWIN with the default configurations of our baselines. All OPTWIN configurations had $\delta=0.99$, $w_{max} =$ 25,000, and pre-computed values for $\nu$, $t\_ppf$, and $f\_ppf$ (as described on Section \ref{sec:implementation}). The difference among the OPTWIN configurations is only on $\rho$, which we varied between $0.1$, $0.5$, and $1.0$ to better understand how our robustness parameter affects OPTWIN's performance in practice.

%explain ``Concept Drift'' configuration
We performed two types of experiments on MOA. The first one uses the ``Concept Drift'' interface, in which MOA creates a stream of data points (either binary or non-binary) and produces a concept drift that can be sudden or gradual. We later refer to those experiments according to their data input and their drift type.%as ``gradual binary drift'', ``gradual non-binary drift'', ``sudden binary drift'' and ``sudden non-binary drift''. 

%explain ``Classification'' configuration
The second type of experiment uses the ``Classification'' interface. It generates data streams based on synthetic datasets (STAGGER, RANDOM RBF, and AGRAWL) \cite{schlimmer1986incremental,bifet2009new,agrawal1993database} and real-world ones (Electricity and Covertype) \cite{blackard1999comparative,harries1999splice}. The idea of these experiments is to train a classifier that is reset every time a concept drift is detected by a drift detector. We chose MOA's built-in Naive Bayes (NB) classifier for its simplicity, which facilitates the analysis of the drift-detection results. For the synthetic datasets, we generate data streams with 100,000 data points with drifts occurring every 20,000 data points (either sudden or gradual). For the real-world data sets, the drifts are already present and have an unknown location on the stream.

%introduce experiment on Table 1
Table \ref{tb:false_positive} presents the comparison among drift detectors on the above-mentioned configurations. We repeated each experiment 30 times and compared their average TP, FP and FN rates to compute their micro-average precision, recall, and F1-score, along with their average drift-detection delay (in terms of the number of streamed elements between the occurrence of a known concept drift and its identification by the detector). Note that we did not include in Table \ref{tb:false_positive} the ``Classification'' experiments on real-world datasets nor the ones with gradual concept drifts. For the real-world datasets, it is not possible to calculate the above-mentioned metrics without knowing the drift's locations. For the gradual drifts, we observed a divergence between the starting and ending points of those drifts in the MOA documentation and in practice. Therefore, we did not include those configurations in our comparison. 

{
\setlength{\abovecaptionskip}{-12pt}
\small
\begin{table}
\centering
\begin{tabular}{l l c c c c c}
\hline
\textbf{Experiment} & \textbf{Drift Detector} & \textbf{Delay} & \textbf{FP} & \textbf{P} & \textbf{R} & \textbf{F1} \\
& ADWIN & 280 & 16.33 & 43\% & 100\% & 60\% \\
& DDM & 365 & 0.37 & 88\% & 100\% & 93\%\\
gradual & EDDM & 148 & 6.33 & 56\% & 100\% & 71\% \\
binary & STEPD & 180 & 8.00 & 23\% & 100\% & 37\% \\
drift & ECDD & \textbf{117} & 5.37 & 27\% & 100\% & 42\% \\
& OPTWIN $\rho=0.1$ & 328 & 0.30 & 88\% & 100\% & 94\% \\
& OPTWIN $\rho=0.5$ & 278 & 0.10 & 96\% & 100\% & 98\% \\
& OPTWIN $\rho=1.0$ & 317 & 0.07 & 97\% & 100\% & \textbf{99}\% \\
\hline
& ADWIN & 145 & 0.00 & 100\% & 100\% & \textbf{100}\% \\
gradual & STEPD & 41 & 150 & 10\% & 100\% & 18\% \\
non-binary & OPTWIN $\rho=0.1$ & \textbf{2.00} & 0.00 & 100\% & 100\% & \textbf{100}\% \\
drift& OPTWIN $\rho=0.5$ & \textbf{2.00} & 0.00 & 100\% & 100\%  & \textbf{100}\% \\
& OPTWIN $\rho=1.0$ & \textbf{2.00} & 0.00 & 100\% & 100\% & \textbf{100}\% \\
\hline
& ADWIN & 46.33 & 1.87 & 35\% & 100\% & 52\% \\
& DDM & 64.50 & 0.20 & 83\% & 100 & 91\%\\
sudden & EDDM & 26.77 & 6.57 & 13\% & 100\% & 23\% \\
binary & STEPD & \textbf{0.40} & 6.67 & 71\% & 100\% & 83\% \\
drift & ECDD & 5.47 & 2.67 & 27\% & 97\% & 42\% \\
& OPTWIN $\rho=0.1$ & 75.13 & 0.00 & 100\% & 100\% & \textbf{100}\% \\
& OPTWIN $\rho=0.5$ & 28.17 & 0.00 & 100\% & 100\% & \textbf{100}\% \\
& OPTWIN $\rho=1.0$ & 18.33 & 0.33 & 75\% & 100\% & 86\% \\
\hline
& ADWIN & 25.00 & 2.00 & 33\% & 100\% & 50\% \\
sudden & STEPD & 21.00 & 32.00 & 3\% & 100\% & 6\% \\
non-binary & OPTWIN $\rho=0.1$ & \textbf{1.00} & 0.00 & 100\% & 100\% & \textbf{100}\% \\
drift& OPTWIN $\rho=0.5$ & \textbf{1.00} & 0.00 & 100\% & 100\%  & \textbf{100}\% \\
& OPTWIN $\rho=1.0$ & \textbf{1.00} & 0.00 & 100\% & 100\% & \textbf{100}\% \\
\hline
& ADWIN & 31.00 & 0.30 & 93\% & 100\% & 96\% \\
& DDM & 6.33 & 0.17 & 96\% & 100\% & 98\% \\
sudden & EDDM & 40.01 & 0.00 & 100\% & 100\% & \textbf{100}\% \\
STAGGER & STEPD & 17.39 & 31.40 & 11\% & 99\% & 20\% \\
& ECDD & 0.72 & 0.47 & 90\% & 100\% & 94\% \\
& OPTWIN $\rho=0.1$ & 0.76 & 0.27 & 94\% & 100\% & 97\% \\
& OPTWIN $\rho=0.5$ & \textbf{0.72} & 0.43 & 90\% & 100\% & 95\% \\
& OPTWIN $\rho=1.0$ & \textbf{0.72} & 0.60 & 87\% & 100\% & 93\% \\
\hline
& ADWIN & 169.67 & 6.00 & 33\% & 75\% & 46\%\\\
& DDM & 536.33 & 2.00 & 60\% & 75\% & 67\% \\
sudden & EDDM & \textbf{53.55} & 11.00 & 21\% & 75\% & 33\% \\
RANDOM & STEPD & 281.25 & 25.00 & 14\% & 100\% & 24\% \\
RBF & ECDD & 71.75 & 174.00 & 2\% & 100\% & 4\% \\
& OPTWIN $\rho=0.1$ & 315.00 & 0.00 & 100\% & 75\% & \textbf{86}\% \\
& OPTWIN $\rho=0.5$ & 187.00 & 0.00 & 100\% & 75\% & \textbf{86}\% \\
& OPTWIN $\rho=1.0$ & 1,931.50 & 1.00 & 67\% & 50\% & 57\% \\
\hline
& ADWIN & \textbf{229.40} & 4.23 & 49\% & 100\% & 65\% \\
& DDM & 1,875.87 & 0.90 & 78\% & 80\% & 79\% \\
sudden & EDDM & 5,370.47 & 17.20 & 12\% & 60\% & 20\% \\
AGRAWAL & STEPD & 838.03 & 23.47 & 14\% & 99\% & 25\% \\
& ECDD & 465.90 & 153.57 & 3\% & 100\% & 5\% \\
& OPTWIN $\rho=0.1$ & 371.62 & 0.63 & 86\% & 100\% & \textbf{93}\% \\
& OPTWIN $\rho=0.5$ & 350.89 & 0.77 & 83\% & 93\% & 88\% \\
& OPTWIN $\rho=1.0$ & 630.63 & 0.27 & 93\% & 88\% & 91\% \\
\hline
\end{tabular}
\caption{Statistics of drift identification on synthetic datasets.}
\label{tb:false_positive}
\end{table}
}

%Discuss Table 1 results
Based on the results in Table \ref{tb:false_positive}, we can generally observe a high F1-score for OPTWIN when compared to the baselines. In fact, with $\rho \leq 0.5$, OPTWIN's average F1-score is over 95\%, followed by OPTWIN with $\rho=1.0$ achieving 89,2\%, DDM with 89,7\%, ADWIN reaching 67\% and the other detectors less than 50\%. We assert this due to OPTWIN's low FP rate which produces a high precision and F1-score, respectively. We further compared the F1-scores of all configurations of OPTWIN with the two drift detectors that can be used for regression problems (ADWIN and STEPD), which showed OPTWIN to be superior based on a one-tailed Wilcoxon signed-rank test with $\alpha=0.05$ in a statistically significant manner. 

Regarding the drift-detection delay, OPTWIN with $\rho = 0.5$ is the drift detector with the smallest delay, taking on average 121 iterations to detect a concept drift; followed by ADWIN, ECDD, and OPTWIN at $\rho = 0.1$ taking 132, 132 and 156 iterations each; the other detectors took on average between 198 and 1127 iterations to detect a drift, with OPTWIN at $\rho = 1.0$ taking 414 on average. Observe that, the higher the FP rate of a drift detector, the higher are also its chances of identifying a drift earlier. Therefore, when analyzing ECDD's average drift delay of 132 iterations, we have to take into consideration that it had an average of 67 FPs per run, in contrast to an average of less than 0.4 for any of the OPTWIN configurations. Furthermore, considering that DDM, EDDM, and ECDD depend on binary input data, they were not included in the experiments using the ``non-binary'' datasets.

We can better visualize the difference between the drift detectors in Figures \ref{fig:abrupt} and \ref{fig:gradual}, which represent one of the 30 runs of the ``sudden binary drift'' and the ``gradual binary drift'' configurations, respectively (we selected the runs with results closest to the ones on the observed average). In Figure \ref{fig:abrupt}, we can see the relatively high FP rate of the EDDM, ADWIN and ECDD detectors when compared to OPTWIN, DDM and STEPD. Moreover, we can see that OPTWIN's detection delay decreases as $\rho$ increases. In Figure \ref{fig:gradual}, we cannot observe the same effect of $\rho$ in OPTWIN's delay detection. Nevertheless, we can still observe the high FP rate of EDDM, ECDD and ADWIN compared to the other drift detectors. We note that STEPD's high FP rate comes from a few runs with dozens of FPs.

{
\setlength{\belowcaptionskip}{-15pt}
\setlength{\abovecaptionskip}{-10pt}
\begin{figure}
\setlength{\columnsep}{0.1\columnsep}
\setlength{\subfigtopskip}{0.1\subfigtopskip}
\setlength{\subfigbottomskip}{0.1\subfigbottomskip}
\setlength{\subfigcapskip}{0.1\subfigcapskip}
\begin{multicols}{2}
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/sudden_drift/abr_b_optwin0.1.png}} \\
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/sudden_drift/abr_b_optwin0.5.png}} \\
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/sudden_drift/abr_b_optwin1.0.png}} \\
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/sudden_drift/abr_b_adwin.png}} \\
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/sudden_drift/abr_b_ddm.png}} \\
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/sudden_drift/abr_b_eddm.png}} \\
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/sudden_drift/abr_b_stepd.png}} \\
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/sudden_drift/abr_b_ecdd.png}} \\
\end{multicols}
\caption{Sudden binary drift detection with average FP rates compared to drift-detection delays.}
\label{fig:abrupt}
\end{figure}
}

{
\setlength{\belowcaptionskip}{-15pt}
\setlength{\abovecaptionskip}{-10pt}
\begin{figure}
\setlength{\columnsep}{0.1\columnsep}
\setlength{\subfigtopskip}{0.1\subfigtopskip}
\setlength{\subfigbottomskip}{0.1\subfigbottomskip}
\setlength{\subfigcapskip}{0.1\subfigcapskip}
\begin{multicols}{2}
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/gradual_drift/grad_b_optwin0.1.png}} \\
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/gradual_drift/grad_b_optwin0.5.png}} \\
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/gradual_drift/grad_b_optwin1.0.png}} \\
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/gradual_drift/grad_b_adwin.png}} \\
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/gradual_drift/grad_b_ddm.png}} \\
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/gradual_drift/grad_b_eddm.png}} \\
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/gradual_drift/grad_b_stepd.png}} \\
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/gradual_drift/grad_b_ecdd.png}} \\
\end{multicols}
\caption{Gradual binary drift detection with average TP and FP rates compared to drift-detection delays.}
\label{fig:gradual}
\end{figure}
}

In Figure \ref{fig:agrawl}, we can once again see OPTWIN and DDM identifying all the drifts with a low FP rate. However, in this scenario, ADWIN also produces only a few FPs, which we noticed to occur immediately after correctly identifying a concept drift. This is due to the time it takes to adapt its window size and remove data points from before the concept drift. In this use case, ECDD and STEPD produce almost ``random guesses'' on the location of the concept drifts. 

{
\setlength{\abovecaptionskip}{-10pt}
\setlength{\belowcaptionskip}{-18pt}
\begin{figure}
\setlength{\columnsep}{0.1\columnsep}
\setlength{\subfigtopskip}{0.1\subfigtopskip}
\setlength{\subfigbottomskip}{0.1\subfigbottomskip}
\setlength{\subfigcapskip}{0.1\subfigcapskip}
\begin{multicols}{2}
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/agrawl/agrawl_optwin0.1.png}} \\
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/agrawl/agrawl_optwin0.5.png}} \\
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/agrawl/agrawl_optwin1.0.png}} \\
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/agrawl/agrawl_adwin.png}} \\
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/agrawl/agrawl_ddm.png}} \\
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/agrawl/agrawl_eddm.png}} \\
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/agrawl/agrawl_stepd.png}} \\
    \subfigure{\includegraphics[width=1\columnwidth]{Figures/agrawl/agrawl_ecdd.png}} \\
\end{multicols}
\caption{TP and FP rates for drift detection on the AGRAWAL dataset with sudden concept drifts.}
\label{fig:agrawl}
\end{figure}
}

\subsection{Classification Experiments}

In the ``Classification'' experiments (still using MOA as platform), we can analyze the average accuracy achieved by the NB classifier when varying the drift detectors (cf. Table \ref{tb:adaptation_sudden}). The idea is that the better a drift detector's performance, the better the classifier can adapt to the concept drifts, thus generating a higher prediction accuracy. However, the fast and accurate detection of the drifts did not always traverse to a better accuracy for the classifier. We can observe this by comparing Tables \ref{tb:false_positive} and \ref{tb:adaptation_sudden}, in which experiments using drift detectors that produced a low F1-score in Table \ref{tb:false_positive} achieved good accuracy in Table \ref{tb:adaptation_sudden}. Moreover, the drift detectors with the best accuracy on real-world data sets were the ones that detected more drifts, which is why ECDD achieved such good accuracy (being the detector that produced the higher amount of FPs). For example, ECDD detected 426 drifts on the Electricity dataset---more than twice as many as all other drift detectors. 

{
\small
\setlength{\abovecaptionskip}{-15pt}
\begin{table*}
\centering
\begin{tabular}{ l | c c c | c c c | c c }
& \multicolumn{3}{c}{Sudden drift} & \multicolumn{3}{c}{Gradual drift} & \multicolumn{2}{c}{Real-world datasets} \\
Drift Detector & STAGGER & Random RBF & AGRAWAL & STAGGER & Random RBF & AGRAWAL & Electricity & Covertype \\
\hline
No drift detector & 66.31 & 58.69 & 57.94 & 66.31 & 58.69 & 57.93 & 73.36 & 60.52 \\
ADWIN & 99.89 & 69.74 & \textbf{70.22} & 98,78 & 69,48 & 69,89  & 80.01 & 82.49\\
DDM & \textbf{99.96} & 68.18 & 65.53 & 98,67 & 68,19 & 65,80 & 81.18 & 88.03\\
EDDM & 99.87 & 65.99 & 65.46 & \textbf{98,83} & 66,92 & 65,31 & 84.83 & 86.08\\
STEPD & 98.74 & \textbf{70.92} & 69.48 & 98,78 & \textbf{70,49} & 69,13 & 84.49 & 87.53\\
ECDD & \textbf{99.96} & 68.64 & 67.03 & 98,71 & 68,52 & 66,80 & \textbf{86.76} & \textbf{90.16}\\
OPTWIN $\rho=0.1$ & \textbf{99.96} & 69.65 & 70.11 & 98,72 & 69,54 &  \textbf{69,94} & 79.99 & 83.29\\
OPTWIN $\rho=0.5$ & \textbf{99.96} & 69.77 & 69.91 & 98,51 & 69,48 &  69,27 & 83.30 & 85.63\\
OPTWIN $\rho=1.0$ & \textbf{99.96} & 68.67 & 69.44 & 98,36 & 68,48 &  68,61 & 82.96 & 86.31\\
\end{tabular}
\caption{Accuracy of NB on synthetic and real-world datasets.}
\label{tb:adaptation_sudden}
\end{table*}
}

\subsection{Neural Network Experiments}

To further explore OPTWIN's behavior in a regression scenario, we compared it with ADWIN for identifying drifts from the loss of a CNN. We chose ADWIN as our baseline because it was the drift detector with the best F1-score among the ones that do not require binary inputs (thus excluding DDM, EDDM and ECDD). To simplify the reader's understanding of the generation of the concept drift, instead of training a regression problem on a CNN, we here focused on image classification by swapping the labels of the images. Thus, we provoked 4 concept drifts by swapping the labels of two classes of images every 20\% of the simulated data stream. For example, after 62,480 iterations, we swapped the labels between images from ``cats'' to ``horses''. Nevertheless, as the variable tracked by the drift detectors is the loss of the CNN, the type of the problem or the network architecture should not affect the experiment.

We pre-trained an image classification model \cite{tensorflow_2022} using the CIFAR-10 \cite{krizhevsky2009learning} data set during 100 epochs, achieving an average of 89\% training accuracy over 3 different runs. Then, we simulated an OL scenario with concept drifts. Our data stream was formed by batches of 32 images from the CIFAR-10 dataset; with a total of 312,400 data points (equivalent to 100 epochs). We simulated our 4 concept drifts by swapping the labels of two classes every 62,480 iterations (the equivalent of 20 epochs). At every iteration, the model classified the 32 images and outputted the loss of the batch. We inputted this loss into the drift-detection algorithm. If a drift was detected, the next 9,372 batches of images (the equivalent of 3 epochs) were used for fine-tuning the model (thus adapting it to the concept drift). Therefore, the goal was for the drift detector to identify the 4 concept drifts that we simulated, triggering the fine-tuning of the model for a total of 12 epochs (3 epochs per drift).

In Figure \ref{fig:cifar}, we compare OPTWIN and ADWIN under the setting described above. First, we note that ADWIN's high FP rates made it retrain the model for much longer than OPTWIN. In comparison, ADWIN identified 15 concept drifts (with 11 FPs), thus triggering model fine-tuning for 61,562 iterations which took in total 945 seconds. In contrast, OPTWIN identified just 5 drifts (with 1 FP), thus triggering the model fine-tuning for 23,430 iterations which took 781 seconds. We note that OPTWIN's running time per iteration is superior to ADWIN, $1e^{-5}$ against $6e^{-6}$ seconds. However, OPTWIN still ends up speeding up the OL pipeline whenever retraining is triggered by the concept-drift detection (21\% faster in this use case). This is because the training of a learner is usually computationally more expensive than the drift detection. Thus, with fewer FPs, the total training time can be reduced substantially.

{
\setlength{\belowcaptionskip}{-15pt}
\setlength{\abovecaptionskip}{-10pt}
\begin{figure}
\setlength{\columnsep}{0.1\columnsep}
\setlength{\subfigtopskip}{0.1\subfigtopskip}
\setlength{\subfigbottomskip}{0.1\subfigbottomskip}
\setlength{\subfigcapskip}{0.1\subfigcapskip}
\begin{multicols}{2}
    \subfigure{\includegraphics[width=.98\columnwidth]{Figures/cifar_optwin.png}} \\
    \subfigure{\includegraphics[width=.98\columnwidth]{Figures/cifar_adwin.png}} \\
\end{multicols}
\caption{Sudden drift detection over the loss of a NN.}
\label{fig:cifar}
\end{figure}
}
